Parameterized Fast and Safe Tracking (FaSTrack) using Deepreach

Fast and Safe Tracking (FaSTrack) is a modular framework that provides safety guarantees while planning and executing trajectories in real time via value functions of Hamilton-Jacobi (HJ) reachability. These value functions are computed through dynamic programming, which is notorious for being computationally inefficient. Moreover, the resulting trajectory does not adapt online to the environment, such as sudden disturbances or obstacles. DeepReach is a scalable deep learning method to HJ reachability that allows parameterization of states, which opens up possibilities for online adaptation to various controls and disturbances. In this paper, we propose Parametric FaSTrack, which uses DeepReach to approximate a value function that parameterizes the control bounds of the planning model. The new framework can smoothly trade off between the navigation speed and the tracking error (therefore maneuverability) while guaranteeing obstacle avoidance in a priori unknown environments. We demonstrate our method through two examples and a benchmark comparison with existing methods, showing the safety, efficiency, and faster solution times of the framework.

==> sections/deepreach.tex <==
DeepReach is a recently proposed neural PDE solver that mitigates the ``curse of dimensionality'' in HJ reachability analysis. Given a set of parameters $\theta$, a deep neural network (DNN) is trained  to approximate the value function $V_\theta(x,t)$, instead of solving the HJI-VI directly. This process bypasses the dimensionality of a system and its grid parameters, which significantly improves computation time. Since the HJI-VI is not directly solved, there is a possibility that the ground truth value function may not be learned. To address this issue, the HJI-VI is defined as a loss term during to guide the training.
Probabilistic safety guarantees for DeepReach can be determined through a scenario optimization approach: by sampling M states with the algorithm, this method finds the violation rate of the trained value function within a defined number of iterations or a violation threshold $\epsilon$.
% By inputting the time and state of the given system, the DNN outputs the trained value function. 

Parameter-conditioned reachability (PCR) assumes that the uncertainty acting on the system can be represented as a disturbance $d$, where the disturbance bound is parameterized by $\beta$, i.e. $d \in\left[\underline{d}\left(\beta_d\right), \bar{d}\left(\beta_d\right)\right]$.  This term $\beta$ is then treated as a virtual state in the system model. Though this virtual state has no dynamics, it allows the DNN to learn various value functions simultaneously, producing a parameterized value function $V(x,\beta)$. PCR effectively diminishes separate training needs for value functions corresponding to the changed system, and solves them in the same fashion as DeepReach, which also allows for a swift computation time of high dimensional systems. 
% In traditional reachability frameworks, the ability to parameterize value functions was not possible. Training value functions with different control, disturbance, or environmental parameters would require individual training of the value functions, which would require significantly more time due to the computational time associated with it. Parameter-Conditioned Reachability effectively diminishes separate training needs for various value functions, adding onto the benefits of DeepReach for high dimensional systems.
A system can leverage the effectiveness of PCR online by taking into account any sudden changes in disturbance bounds or the environment. Its online adaptability improves a system's robustness by maintaining its safety while decreasing the solution time. The optimal control can be determined from the gradients of the learned value function.

%The parameter-conditioned loss function for training the DNN is denoted by the following:
%\begin{align*}
%    h(x_i,t_i,\beta_i;\theta) &= h_1(x_i,t_i,\beta_i;\theta)+\lambda h_2(x_i,t_i,\beta_i;\theta),\\
%    h_1(x_i,t_i,\beta_i;\theta) &= \left|\left|V_\theta(x_i,t_i;\beta_i) - l(x_i;\beta_i)\right|\right|_{(t_i = T)},\\
%    h_2(x_i, t_i,\beta_i;\theta) &= \left|\left|\max\{D_tV_\theta(x_i,t_i;\beta_i) + H(x_i,t_i;\beta_i),\, l(x_i;\beta_i) - V_\theta(x_i,t_i;\beta_i)\}\right|\right|.
%\end{align*}
%Here, each loss term represents the parameterized value function and the RHS of HJI-VI \eqref{eqn:HJIVI}. $h_1(\cdot)$ is the difference between the parameterized value function, $V_\theta(x_i,t_i;\beta_i)$, and the boundary condition, $l(x_i;\beta_i)$, which ultimately represents the ground truth value function. This allows the DNN propogate the value function correctly when training, ensuring that the wrong value function is not learned for the respective $\beta$ values. $h_2(\cdot)$ guides the DNN to train the parameterized value function consistent with the HJI-VI. The HJI-VI is a necessary term, since reachability solutions are derived from the HJI-VI. Finally, $h(\cdot)$ weighs $h_1(\cdot)$ and $h_2(\cdot)$ via $\lambda$ to determine the importance between the HJI-VI and the ground truth value function.


% \begin{lemma}
%     the value function computed from the deepreach is a strict over approximation of the HJ value function. 
%     \zgnote{or should we say the minimal level set of the deepreach function is a strict over approximation of the minmal level set of the original HJ value function}
% \end{lemma}


==> sections/fastrack_text.tex <==
In this section we introduce the offline precomputation and online algorithm for FaSTrack.  The offline subsection provides an overview of computing the TEB (tracking error bound) that bounds the relative distance between the simple model used for online planning and the more sophisticated model of the true system.  The online subsection explains how this bound is used to ensure safety of the system when planning online using a simplified planning model of the system.
%To compute the TEBs we use the FaSTrack framework described in \cite{Herbert2017}, wherein the maximum tracking error between a high-dimensional tracking model of the system and a low-dimensional planning model of the system is computed.  In this section we define the tracking and planning models, their relative dynamics, and set up the offline computation to generate the TEB between the tracking model of the true system and each planning model employed by the meta-planner. \shnote{also we show online fastrack stuff}.

\subsection{Offline Computation for FaSTrack}
\subsubsection{Tracking Model}
\label{subsec:tracking_model}

The tracking model should be a realistic representation of the real system dynamics, and in general may be nonlinear and high-dimensional. Let $\tstate\in \tset\subseteq\R^{n_s}$ represent the state variables of the tracking model. The evolution of the dynamics satisfies the ordinary differential equation (ODE): 

\begin{equation}
\begin{aligned}
\label{eq:tdyn}
\frac{d\tstate}{d\tvar} = \dot{\tstate} = \tdyn(\tstate(\tvar), \tctrl(\tvar), \dstb(\tvar)), \tvar \in [0, \thor], \\
\tstate(\tvar) \in \tset, \tctrl(\tvar) \in \tcset, \dstb(\tvar) \in \dset,
\end{aligned}
\end{equation}
We assume that the tracking model dynamics $\tdyn : \tset\ \times\ \tcset \times \dset \rightarrow \tset$ are uniformly continuous and Lipschitz continuous in the system state $\tstate$ for a fixed control and disturbance functions $\tctrl(\cdot), \dstb(\cdot)$. 
At every time $t$, the control $\tctrl$ is constrained by the compact set $\tcset\subseteq \R^{n_{u_s}}$, and the disturbance $\dstb$ is constrained by the compact set $\dset\subseteq \R^{n_d}$.
Furthermore, the control function $\tctrl(\cdot)$ and disturbance function $\dstb(\cdot)$ are measurable functions of time:
\begin{equation}
\begin{aligned}
\tctrl(\cdot) \in \tcfset(t) = \{\phi: [0, \thor] \rightarrow \tcset: \phi(\cdot) \text{ is measurable}\}\\
\dstb(\cdot) \in \dfset(t) = \{\phi: [0, \thor] \rightarrow \dset: \phi(\cdot) \text{ is measurable}\}
\end{aligned}
\end{equation}
where $\tcfset$ and $\dfset$ represent the set of functions that respectively satisfy control and disturbance constraints at all times. Under these assumptions there exists a unique trajectory solving (\ref{eq:tdyn}) for a given $\tctrl(\cdot) \in \tcset$ \cite{Coddington84}. 

Under these assumptions there exists a unique trajectory solving (\ref{eq:tdyn}) for a given $\tctrl(\cdot) \in \tcfset, \dstb(\cdot)\in\dfset$ \cite{Coddington84}. The trajectories of (\ref{eq:tdyn}) that solve this ODE will be denoted as $\ttraj(\tvar; \tstate, \tvar_0, \tctrl(\cdot), \dstb(\cdot))$, where $\tvar_0,\tvar \in [0, \thor]$ and $\tvar_0 \leq \tvar$. This trajectory notation represents the state of the system at time $\tvar$, given that the trajectory is initiated at state $\tstate$ and time $\tvar_0$ and the applied control and disturbance functions are $\tctrl(\cdot)$ and disturbance $\dstb(\cdot)$ respectively.
These trajectories will satisfy the initial condition and the ODE (\ref{eq:tdyn}) almost everywhere:

\begin{align*}
&\frac{d}{d\tvar}\ttraj(\tvar; \tstate_0, \tvar_0, \tctrl(\cdot), \dstb(\cdot)) = \\ &\qquad \tdyn(\ttraj(\tvar; \tstate_0, \tvar_0, \tctrl(\cdot), \dstb(\cdot)), \tctrl(\tvar), \dstb(\cdot)), \\
&\ttraj(\tvar_0; \tstate_0, \tvar_0, \tctrl(\cdot), \dstb(\cdot)) = \tstate_0.
\end{align*}

For a running example we will consider a tracking model of a simple double-integrator with control $\tctrl$ and disturbances ${\dstb = [\dstb_v, \dstb_{a}]^T}$:
\begin{equation}
\small
\label{eq:tracking_dyn_example}
\begin{aligned}
\begin{array}{c}
\left[
\begin{array}{c}
\dot{\tstate}_x\\
\dot{\tstate}_{vx}\\
\end{array}
\right]
=
\left[
\begin{array}{c}
\tstate_{vx} - d_v\\
\tctrl -d_{a}\\
\end{array}
\right]
\end{array}
\end{aligned}
\end{equation}

\subsubsection{Planning Model}
\label{subsec:planning_model}
Each planning mode must have an associate planning model defining the class of trajectories generated by the planning mode. Let $\pstate$ represent the state variables of the planning model corresponding to planning mode $i$, and let $\pctrli$ be its control. 
We assume that the planning states $\pstatei \in \pseti$ are a subset of the tracking states $\tstate \in \tset$, so that $\pseti$ is a subspace within $\tset$.
This assumption is reasonable since a lower-fidelity model of a system typically involves a subset of the system's states.
The dynamics of the planning model satisfy
\begin{align}
\label{eq:pdyn}
\frac{d\pstatei}{d\tvar} &= \dot{\pstate}^{(i)} = \pdyn(\pstatei, \pctrli), \\
\tvar \in [0, \thor], \quad \pstatei& \in \pseti, \quad \pctrli \in \pcseti,
\end{align}

\noindent with the analogous assumptions on continuity and boundedness as those for \eqref{eq:tdyn}.

The planning algorithm may not directly use a planning model, but generally can be interpreted using a planning model (e.g. geometric paths generated by RRT can be described by a point with direct velocity control).
Note that the planning model does not need a disturbance input. Disturbances need only be considered in the tracking model and not the planning model, since the latter only exists in the abstract as a reference for the former.

\subsubsection{Relative Dynamics}
\label{subsec:relative_dynamics}
The relative system is obtained by fixing the planning model to the origin and finding the dynamics of the tracking model relative to the planning model.
Defining $\rstatei$ to be the relative system state given planning mode $i$, we write

\begin{equation}
\label{eq:rstate}
\rstatei = \rtrans(\tstate,\pstatei)(\tstate - \ptmat\pstatei)
\end{equation}

\noindent where $\ptmat$ matches the common states of $\tstate$ and $\pstatei$ by augmenting the state space of the planning model.
The relative system states $\rstatei$ represent the tracking system states relative to the planning states.
The function $\rtrans$ is a linear transform that simplifies the relative system dynamics to be of the form

\begin{equation}
\label{eq:rdyn}
\dot\rstate^{(i)} = \rdyn(\rstatei, \tctrl, \pctrl, \dstb),
\end{equation}

\noindent which only depends on the relative system state $\rstatei$.
A transform $\rtrans$ that achieves the relative system dynamics in the form of \eqref{eq:rdyn} is often the identity map or the rotation map when the autonomous system is a mobile robot; therefore, in this paper, we assume that a suitable $\rtrans$ is available.

Using our tracking and planning model examples from above we can define the dynamics of a double-integrator tracking a 1D point mass as:%Similarly, $\tpmat$ projects the state space of the tracking model onto the planning model: $\pstate = \tpmat(\tstate-\rstate)$. This will be used to update the planning model in the online algorithm.

\begin{equation}
\small
\label{eq:rdyn_example}
\begin{aligned}
\begin{array}{c}
\left[
\begin{array}{c}
\dot{r}_x\\
\dot{s}_{vx}\\
\end{array}
\right]
=
\left[
\begin{array}{c}
\tstate_{vx} - d_v - \pctrl\\
\tctrl -d_a\\
\end{array}
\right]
\end{array}
\end{aligned}
\end{equation}

\subsubsection{Tracking Error Bound and Safety Controller Computation}
Here we will provide a brief overview of the steps to compute the tracking error bound.  For details on the process, please refer to \cite{chen2020fastrack,Herbert2017}.
To quantify the error between two systems, we first define an error function in the relative state space.  This error function is typically chosen to be the squared distance to the origin (i.e. squared distance of the tracking model to the planning model).
To obtain a bound on error, we compute the highest error over all time that the relative system will ever attain when both players are acting optimally:

\begin{align}
&\mathcal{V}(\rstate,\thor)= \max_{\tvar\in [0, \thor]} \errfunc\Big(\rtraj(\tvar; \rstate, 0, \tctrl^*(\cdot), \pctrl^*(\cdot), \dstb^*(\cdot))\Big). \label{eq:valfunc1}
\end{align} 

In order to determine the optimal tracking control, planning control, and disturbance, we must first determine the information structure, i.e. how and when each agent makes decisions.  We force the tracking model to determine its action first; it will try to minimize the tracking error to track the plan as closely as possible.  To capture the worst possible error over time, we set the planning model and any disturbances to act adversarially by maximizing the error.  Moreover, we allow both to choose their actions second while employing nonanticipative strategies: at each iteration they know the current action of the tracking model, but no future actions.  By making this worst-case assumption, we can have a precomputed safety guarantee on the maximum error that may \textit{ever} occur online. As in \cite{chen2020fastrack,Herbert2017}, we restrict the planning model and disturbance to use nonanticipative strategies $\pctrl \in \Gamma_\pstate(t)$ and $\dstb \in \Gamma_\dstb(t)$

%To quantify these nonanticipative strategies, we define the planning model's strategy as the mapping $\gamma_{\pstate} : \tcset \rightarrow \pcset$ that determines a planning control based on the tracking control, and is restricted to non-anticipative strategies $\gamma_{\pstate} \in \Gamma_\pstate(t)$.
%We similarly define the disturbance strategy $\gamma_{\dstb}: \tcset \rightarrow \dset$, $\gamma_{\dstb} \in \Gamma_\dstb(t)$.

The optimization procedures over the error function produces the value function:
\begin{align}
&V(\rstate,\thor)= \inf_{\tctrl(\cdot) \in \tcfset(t)}
\sup_{\pctrl \in \Gamma_\pstate(t), \dstb \in \Gamma_\dstb(t)}  \big\{ \nonumber \\
&\qquad\qquad \max_{\tvar\in [0, \thor]} \errfunc\Big(\rtraj(\tvar; \rstate, 0, \tctrl(\cdot), \pctrl(\cdot), \dstb(\cdot))\Big)\big\}. \label{eq:valfunc}
\end{align} 

If the control authority of the tracking model is powerful enough to always eventually remain within some distance from the planning model, this value function will converge to an invariant solution for all time, i.e. $\valfunc_\infty(\rstate) := \lim_{\thor\rightarrow\infty} \valfunc(\rstate, \thor)$. 
Because the planning model is user-defined, convergence can often be achieved by tuning the planning model.

The value function can be computed via existing methods in HJ reachability analysis \cite{Mitchell05, Fisac15}.  It can additionally be solved by other tools such as approximate dynamic programming \cite{royo2018classification} and sum-of-squares optimization \cite{singh2018robust}.

The smallest level set corresponding to the value $\underline\valfunc := \min_{\rstate} \valfunc(\rstate,\thor)$ can be interpreted as the smallest possible tracking error of the system. 
The TEB is given by the set\footnote{In practice, since $\valfunc$ is obtained numerically, we set $\TEB(\tau) = \{\rstate: \valfunc(\rstate, \thor - \tau) \le \underline\valfunc + \epsilon\}$ for some suitably small $\epsilon>0$.}

\begin{align} \label{eq:TEB_fin}
\TEB(\tau) = \{\rstate: \valfunc(\rstate, \thor - \tau) \le \underline\valfunc\}.
\end{align}

Note that TEB is only guaranteed if the system uses the corresponding safety controller when on the boundary of the set (i.e. when the tracking model is on the edge of the error bound).  This safety controller is obtained from the value function's spatial gradient \cite{Mitchell05, Fisac15}, $\deriv(\rstate, \tvar)$, as

\begin{align} \label{eq:opt_ctrl_fin}
\tctrl^*(\rstate, \tvar) = \arg\min_{\tctrl\in\tcset} \max_{\pctrl\in\pcset, \dstb\in\dset} \nabla\valfunc(\rstate, \tvar) \cdot \rdyn(\rstate,\tctrl,\pctrl,\dstb)
\end{align}

\subsection{Online Computation for FaSTrack}
The online algorithm for FaSTrack begins by identifying the initial state of the autonomous system as the tracking agent. The planning agent is initialized to be within one TEB bound of the tracking agent.  The planning state is an input to some path or trajectory planning algorithm (e.g. A$^*$, MPC), along with environmental state constraints that are augmented by the TEB (e.g. augmented obstacles).
The path or trajectory planning algorithm uses this information to compute the next state of the planning agent.  Note that since this next state was computed with the augmented constraints in mind, the planning state will never be within one TEB of the state constraints.

The relative state between the new planning state and the current tracking state is determined. If this relative state is on the boundary of the TEB, the precomputed optimal safety control for that state is used to keep the tracking agent within the TEB.  If the relative state is well within the TEB, any control may be used (e.g. LQR, a learning-based policy, or even the same precomputed safety controller).

The key takeaway of this algorithm is that it is a very lightweight wrapper around the user's desired path or trajectory planner.  There is one step of augmenting constraints before inputting into the planner (which is often done anyways), and a second step of looking up the precomputed safety controller when the relative state is close to the boundary of the TEB. The lightweight nature of this algorithm allows for very fast online planning with the planning agent while maintaining safety with respect to the more sophisticated tracking agent.

==> sections/parametric_fastrack.tex <==
We now introduce the parameterized FaSTrack framework. 
%In Parametric FaSTrack, the offline computation is similar to that of FaSTrack. However,
%This is achieved by parameterizing the value function of FaStrack using the virtual parameter states. 
Figure~\ref{fig:2} visualizes flowcharts representing the offline procedure (left) and the online procedure (right). The components from the original FaSTrack framework are showns in blue, whereas components of our parametric FaSTrack are shown in orange. In this section we will introduce the offline procedure.

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{figures/totalframework.png}
    \caption{Left figure denotes the offline framework (performed once), and the right figure denotes the online framework (performed every iteration). Components of FaSTrack are shown in blue, while components of Parametric FaSTrack are shown in orange.\vspace{-1.5em}}
    \label{fig:2}
\end{figure}

\noindent \textbf{Tracker Model. }In the FaSTrack framework, the \textit{tracker model} represents the true robot and a \textit{planner model} is used for real-time path planning. 
The \textit{tracker model} is given by the following ordinary differential equation (ODE)
\begin{align} \label{eq:tdyn}
    \frac{d \tstate}{d\tvar} =\dot \tstate  = \tdyn ( \tstate (\tvar),\tctrl (\tvar),\dstb (\tvar)  ), \quad \tvar \in [0,\thor], \quad \tstate \in \tset \subset \mathbb R^{n_s},\tctrl \in \tcset \subset \mathbb R^{n_u},\dstb \in \dset \subset \mathbb R^{n_d},
\end{align}
where $\tvar$ is the time and $\tstate$, $\tctrl$ and $\dstb$ are the tracker state, control and disturbance at a given time respectively, with $\tcset$ and $\dset$ to be compact sets. $\tctrl (\cdot) \in \tcfset$ and $\dstb (\cdot) \in \dfset$ are the control and disturbance signal, assumed to be measurable: $\tctrl (\cdot): [0,\thor]\mapsto \tcset$ and $\dstb (\cdot): [0,\thor]\mapsto \dset$.
% \begin{align*}
%     \tctrl (\cdot) \in \tcfset &:= \{ \phi: [0, \thor] \mapsto \tcset , \phi(\cdot) \text{ is measurable} \} ,\\
%     \dstb (\cdot) \in \dfset &:= \{ \phi: [0, \thor] \mapsto \dset , \phi(\cdot) \text{ is measurable}\}.
% \end{align*}
We further assume the dynamics $\tdyn : \tset \times \tcset \times \dset \mapsto \tset$ is Lipschitz continuous in $\tstate$ for fixed $\tctrl (\cdot)$ and $\dstb (\cdot)$. Under these assumptions, a unique solution of \eqref{eq:tdyn} can be solved, denoted as $\ttraj (t; 0, \tstate, \tctrl (\cdot),\dstb(\cdot))$, or in short $\ttraj (t)$. %Denote the goal set as $\mathcal G \subset \tset$ and constraints set $\mathcal C  \subset \tset$. In the paper, $\mathcal C$ denotes the obstacle that the tracker must avoid. 

\noindent \textbf{Planner Model.} The \textit{planner model} is a virtual model designed for path planning, given by the following ODE 
\begin{align*}
    \frac{d \pstate}{ dt} = \dot \pstate = \pdyn(\pstate,\pctrl), \quad \tvar \in [0,\thor], \quad \pstate \in \pset \subset \mathbb R^{n_p}, \pctrl \in \pcset,
\end{align*}
where $\pstate$ is the planner state and $\pctrl$ is the planner control. We assume the planner state is a subset of the tracker state, and the planner space is a subspace of the tracker space. 


Since the path planning is done using the planner model, the goal and constraints sets in the planner space are required. We denote them as $\mathcal G_p$ and $\mathcal C_p$ respectively. Also, since we assume unknown environment and limited sense range, we denote the sensed environment as $\mathcal C_{p,\text{sense}}(t)$, and the augmented obstacle as $\mathcal C_{p,\text{aug}}(t)$. Note both $\mathcal C_{p,\text{sense}}(t)$ and $\mathcal C_{p,\text{aug}}(t)$ are time-varying sets that update at each iteration of planning.  

%\subsubsection{Relative Dynamics}
\noindent \textbf{Relative Dynamics.} The FaSTrack framework provides guarantees by precomputing the maximum error (i.e. distance) possible between the tracker model and planner model. In order to compute this, the \textit{relative dynamics} between the two systems must be determined.
Since the planner space is a subspace of the tracker space, we can always find a matrix $\ptmat \in \mathbb R^{n_s \times n_p}$, and assume we can also find a linear tranformation $\rtrans(\tstate,\pstate)$ s.t. $\rstate = \rtrans(\tstate,\pstate) (\tstate -\ptmat \pstate)$ and 
\begin{align*}
    \dot \rstate = \rdyn (\rstate, \tctrl,\pctrl, \dstb), 
\end{align*}
with solution $\rtraj (t;0,\rstate, \tctrl, \pctrl ,\dstb)$. We denote the common states in tracker and planner as $e$ and the rest as $\eta$, i.e. $\rstate = [e,\eta]$. 

\vspace{2mm}
\noindent \textit{Running example: }consider the tracker model as a unicycle  with controls $\omega$ and $\alpha$:  
\begin{align*}
    \dot  \tstate_1 = \tstate_4 \sin (\tstate_3), \hspace{2mm}
    \dot  \tstate_2 = \tstate_4 \cos (\tstate_3), \hspace{2mm}
    \dot  \tstate_3 = \omega, \hspace{2mm}
    \dot  \tstate_4 = \alpha, 
\end{align*}
% \textit{ with $s = [x,y,\theta,v]$, $x$ position, $y$ position, heading angle and velocity.}
Consider the planning model: 
$\dot  \pstate_1 = u_{px}, \hspace{2mm}
    \dot  \pstate_2 = u_{py},$
where $u_{px}$ and $u_{py}$ are planning controls. Given linear transformation $\rtrans = I_4$ and matrix $\ptmat = \begin{bmatrix} 1&0&0&0 \\ 0&1&0&0\end{bmatrix}^T$, the relative model is:
\begin{align} \label{eq:ex_dubins}
    \dot \rstate_1 = \rstate_4 \sin (\rstate_3) - u_{px}, \hspace{2mm}\dot \rstate_2 = \rstate_4 \cos (\rstate_3 ) - u_{py}, \hspace{2mm}\dot \rstate_3 = \omega, \hspace{2mm}\dot \rstate_4 = \alpha.
\end{align}


\noindent \textbf{Parameterized Relative System.} \shnote{transition sentence} the parameterized relative system for our running example:
\begin{align*}
    \dot r_1 = r_4 \sin (r_3) - u_{px}, \hspace{2mm}\dot r_2 = r_4 \cos (r_3) - u_{py}, \hspace{2mm}\dot r_3 = \omega, \hspace{2mm}\dot r_4 = \alpha, \hspace{2mm}\dot r_5 = 0, \hspace{2mm}\dot r_6 = 0,
\end{align*}

Here, the first 4 states of the relative system are identical to \eqref{eq:ex_dubins}. The control bounds are given as $r_3 \in [-5, 5]$ and $r_4 \in [-1, 1]$. We add $\dot r_5 = u_{px}$ and $\dot r_6 = u_{py}$ as the virtual parameter states with 0 dynamics. These virtual parameter states represent the planner velocity value, $r_5 = \beta_1$ and $r_6 = \beta_2$. The bounds of the planner velocity are given as $u_{px} \in [0.5 \leq \beta_1 \leq 1.25]$ and $u_{py} \in [0.5 \leq \beta_2 \leq 1.25]$. Note that the parameter states can be queried anywhere from the lower bound to the upper bound. 
%\subsubsection{Tracking Error Bound and Safety Controller Computation}
% Key is to introduce HJI-VI / Hamiltonian in this section. Important when introducing loss functions for DeepReach, as it relies on this.

\noindent \textbf{Cost Function.} With the relative dynamics in hand, the maximum possible relative distance (i.e. \textit{tracking error bound}, or TEB) between the two models can be computed.  The error function of this game is denoted as $\ell (\rstate)$, and is chosen to be the Euclidean norm in the relative state space (here, low error corresponds to accurate tracking). We assume that the tracker model will seek to minimize this tracking error by \textit{pursuing} the planner model. 
 Because the environment and therefore behavior of the planner model is unknown \textit{a priori}, to provide safety guarantees we must assume  worst-case actions of the planner model.  This amounts to assuming the planner model is actively seeking to maximize the tracking error and \textit{evade} the tracker model. We have therefore constructed a pursuit-evasion game between the tracker and planner models. 
 
 \noindent \textbf{Offline Computation of the Tracking Error Bound and Controller.} We define the strategies of the planner and disturbance as mappings: $\gamma _p : \tcset \mapsto \pcset$, $\gamma _d : \tcset \mapsto \dset$ and assume they are restricted to be the non-anticipative strategies $\gamma _p \in \Gamma_p$, $\gamma _d \in \Gamma_d$. The value of the game can be defined as: 
\begin{align} \label{eqn:value function}
    \valfunc (\rstate, \thor) = \sup _{\gamma _p \in \Gamma_p, \gamma _d \in \Gamma_d} \inf _{u_s\in \tcfset} \{ \max_{t\in [0 , \thor]} \ell(\rtraj(t; 0, \rstate, \tctrl (\cdot), \gamma _p(\cdot),\gamma _d(\cdot))) \}.
\end{align}
% This value captures the ``largest'' relative state ever achieved in time horizon $[0,\thor]$, under optimal tracker control, worst case planner control and disturbance, and measured by the error function $\ell(\rstate)$. 
% The level set corresponds to the minimal value $\minval = \min_{\rstate} \valfunc(\rstate,\thor)$ defines a time-varying TEB: the relative states stay inside this set within time horizon $[0,\thor]$.
It has been shown that \eqref{eqn:value function} can be computed by solving the following HJI-VI recursively: 
\begin{align}\label{eqn:HJIVI}
    0 = \max \{ \ell(\rstate) - \valfunc(\rstate, t), \quad \frac{\partial \valfunc}{ \partial t} + \min_{\tctrl\in \tcset} \max_{\pctrl \in \pcset,\dstb \in \dset}  \frac{\partial \valfunc}{ \partial \rstate} \cdot \rdyn(\rstate,\tctrl,\pctrl,\dstb) \}, \quad \valfunc(\rstate, 0) = \ell(\rstate),
\end{align}

The value of at a particular $r,t_f$ corresponds to the largest relative distance, or tracking error, that can occur over the time horizon. The smallest non-empty level set of this function therefore provides the smallest tracking error bound and the set of relatives states for which this bound can be achieved over the time horizon.

In the case where the limit function $\valfunc ^\infty (\rstate) = \lim_{\thor \rightarrow \infty} \valfunc (\rstate, \thor)$ exists, every non-empty level set is a robust control invariant set.  The smallest such set, $\minval^\infty = \min_{\rstate} \valfunc ^\infty (\rstate)$, is called the infinite-time TEB: the relative system will stay inside this set for all $t\geq 0$. Throughout the paper, we assume this limit function exist, though extensions to time-varying error bounds have been successful \cite{}. The infinite-time TEB in the relative space and planner space are denoted by
\begin{align*}
    \TEB^\infty := \{ \rstate : \valfunc^\infty(\rstate) \leq \minval ^\infty \}, \quad \TEB^\infty _e := \{e: \exists \eta \text{ s.t. }\valfunc^\infty(e,\eta) \leq \minval ^\infty \}.
\end{align*}

% The time-varying and infinite-time TEBs in the relative space are denoted by
% \begin{align*}
%     \TEB (\tau) := \{ \rstate : \valfunc(\rstate,\thor - \tau) \leq \minval \}, \quad \TEB^\infty := \{ \rstate : \valfunc^\infty(\rstate) \leq \minval ^\infty \}. 
% \end{align*}
% In the online planning part, the obstacles are augmented in the planner space, therefore the TEBs also need to be projected into the planner space 
% \begin{align*}
%     \TEB_e (\tau) := \{ e: \exists \eta \text{ s.t. }\valfunc(e,\eta,\thor-\tau) \leq \minval \}, \quad \TEB^\infty _e := \{e: \exists \eta \text{ s.t. }\valfunc^\infty(e,\eta) \leq \minval ^\infty \}. 
% \end{align*}

%and the limit function can be obtained by solving the above HJI-VI until the value function converge. 
% Note that the tracking model and relative model share the same control input $\tctrl$, therefore the optimal control of the tracker is the same as the optimal control of the tracker, 
\noindent \textbf{Online Planning and Tracking.} Online, the sensed obstacles are augmented by this error bound projected into the planner state space.  The planning algorithm employs the planning model to determine the next planner state.  The autonomous system (represented by the tracker model) can efficiently compute the optimal tracking control via the relative state between itself and the planner: 

\begin{equation}
    \tctrl^* = \text{argmin}_{\tctrl \in \tcset}\max_{\pctrl \in \pcset,\dstb \in \dset} \frac{\partial \valfunc}{ \partial \rstate} \cdot \rdyn(\rstate,\tctrl,\pctrl,\dstb). \label{eq:tracking_control}
\end{equation}
This process repeats until the system has reached the goal.
% This controller is often overly conservative, and we use the idea of safety filter to enhance performance: only apply this optimal control when the trajectory approaches the boundary of the TEB, and apply performance controller when the trajectory is inside of the TEB.

% \begin{lemma}
%     Larger planner control bonuds corresponds to larger TEB. 
%     \begin{proof}
%     Assume $\pcset _1 \subset \pcset _2 $ and that $\TEB ^\infty _1, \TEB ^\infty _2$ are the corresponding TEBs.  
%     \end{proof}
% \end{lemma}

% \subsubsection{Online Execution}
% One iteration of the online execution contains three steps. 
% First, sense the environment. If obstacle is sensed, it is augmented by the $\TEB_e (\tau)$. Then, the planner block takes the augmented environment and output the planner control $\pctrl$. Finally, the tracker block checks current relative state $\rstate$ and determines the tracker control $\tctrl$ based on its value $\valfunc (\rstate)$ and gradient $\frac{\partial \valfunc}{ \partial \rstate}$. 

\subsection{DeepReach and Parameter-Conditioned Reachability}
DeepReach is a recently proposed neural PDE solver that mitigates the ``curse of dimensionality'' in HJ reachability analysis. Given a set of parameters $\theta$, a deep neural network (DNN) is trained  to approximate the value function $V_\theta(x,t)$, instead of solving the HJI-VI directly. This process bypasses the dimensionality of a system and its grid parameters, which significantly improves computation time. Since the HJI-VI is not directly solved, there is a possibility that the ground truth value function may not be learned. To address this issue, the HJI-VI is defined as a loss term during to guide the training.
Probabilistic safety guarantees for DeepReach can be determined through a scenario optimization approach: by sampling M states with the algorithm, this method finds the violation rate of the trained value function within a defined number of iterations or a violation threshold $\epsilon$.
% By inputting the time and state of the given system, the DNN outputs the trained value function. 

Parameter-conditioned reachability (PCR) assumes that the uncertainty acting on the system can be represented as a disturbance $d$, where the disturbance bound is parameterized by $\beta$, i.e. $d \in\left[\underline{d}\left(\beta_d\right), \bar{d}\left(\beta_d\right)\right]$.  This term $\beta$ is then treated as a virtual state in the system model. Though this virtual state has no dynamics, it allows the DNN to learn various value functions simultaneously, producing a parameterized value function $V(x,\beta)$. PCR effectively diminishes separate training needs for value functions corresponding to the changed system, and solves them in the same fashion as DeepReach, which also allows for a swift computation time of high dimensional systems. 
% In traditional reachability frameworks, the ability to parameterize value functions was not possible. Training value functions with different control, disturbance, or environmental parameters would require individual training of the value functions, which would require significantly more time due to the computational time associated with it. Parameter-Conditioned Reachability effectively diminishes separate training needs for various value functions, adding onto the benefits of DeepReach for high dimensional systems.
A system can leverage the effectiveness of PCR online by taking into account any sudden changes in disturbance bounds or the environment. Its online adaptability improves a system's robustness by maintaining its safety while decreasing the solution time. The optimal control can be determined from the gradients of the learned value function.

%The parameter-conditioned loss function for training the DNN is denoted by the following:
%\begin{align*}
%    h(x_i,t_i,\beta_i;\theta) &= h_1(x_i,t_i,\beta_i;\theta)+\lambda h_2(x_i,t_i,\beta_i;\theta),\\
%    h_1(x_i,t_i,\beta_i;\theta) &= \left|\left|V_\theta(x_i,t_i;\beta_i) - l(x_i;\beta_i)\right|\right|_{(t_i = T)},\\
%    h_2(x_i, t_i,\beta_i;\theta) &= \left|\left|\max\{D_tV_\theta(x_i,t_i;\beta_i) + H(x_i,t_i;\beta_i),\, l(x_i;\beta_i) - V_\theta(x_i,t_i;\beta_i)\}\right|\right|.
%\end{align*}
%Here, each loss term represents the parameterized value function and the RHS of HJI-VI \eqref{eqn:HJIVI}. $h_1(\cdot)$ is the difference between the parameterized value function, $V_\theta(x_i,t_i;\beta_i)$, and the boundary condition, $l(x_i;\beta_i)$, which ultimately represents the ground truth value function. This allows the DNN propogate the value function correctly when training, ensuring that the wrong value function is not learned for the respective $\beta$ values. $h_2(\cdot)$ guides the DNN to train the parameterized value function consistent with the HJI-VI. The HJI-VI is a necessary term, since reachability solutions are derived from the HJI-VI. Finally, $h(\cdot)$ weighs $h_1(\cdot)$ and $h_2(\cdot)$ via $\lambda$ to determine the importance between the HJI-VI and the ground truth value function.


% \begin{lemma}
%     the value function computed from the deepreach is a strict over approximation of the HJ value function. 
%     \zgnote{or should we say the minimal level set of the deepreach function is a strict over approximation of the minmal level set of the original HJ value function}
% \end{lemma}



% \subsection{Formal Safety Assurances for DeepReach}


%%%%%%%%%%%%%%%%





\noindent \textbf{DeepReach Training.} For the running example, the error function $l(r_i, \beta_i)$ is denoted as the euclidean norm between $r_1$ and $r_2$, the relative distance states. The Hamiltonian can be defined as:
\begin{align*}
    H(r,t;\beta) = p_1(r_4 \sin (r_3)) + p_2(r_4 \cos (r_3)) + \beta_1 \left| p_1 \right| + \beta_2 \left| p_2 \right| - \omega \left| p_3 \right| - \alpha \left| p_4 \right|,
\end{align*}

Where $p_1$, $p_2$, $p_3$, and $p_4$ represent the partial derivatives of the value function with respect to $r_1$, $r_2$, $r_3$, and $r_4$ respectively. For control affine systems such as this Dubin's car example, the Hamiltonian can simply be computed analytically through the value function gradients.
The cost function for the running example is defined to contain the relative states:
\begin{align}\label{eq:loss_function}
    h_1(r_i,t_i,\beta_i;\theta) &= \left|\left|V_\theta(r_i,t_i;\beta_i) - l(r_i;\beta_i)\right|\right|_{(t_i = T)},\\
    h_2(r_i, t_i,\beta_i;\theta) &= \left|\left|\min\{D_tV_\theta(r_i,t_i;\beta_i) + H(r_i,t_i;\beta_i),\, l(r_i;\beta_i) - V_\theta(r_i,t_i;\beta_i)\}\right|\right|,\\
        h(r_i,t_i,\beta_i;\theta) &= h_1(r_i,t_i,\beta_i;\theta)+\lambda h_2(r_i,t_i,\beta_i;\theta).
\end{align}
Here, each loss term represents the parameterized value function and the RHS of HJI-VI \eqref{eqn:HJIVI}. The term $h_1(\cdot)$ is the difference between the parameterized value function, $V_\theta(x_i,t_i;\beta_i)$, and the boundary condition, $l(x_i;\beta_i)$, which ultimately represents the ground truth value function. This allows the DNN propogate the value function correctly when training, ensuring that the wrong value function is not learned for the respective $\beta$ values. The term $h_2(\cdot)$ guides the DNN to train the parameterized value function consistent with the HJI-VI. The HJI-VI is a necessary term, since reachability solutions are derived from the HJI-VI. Finally, $h(\cdot)$ weighs $h_1(\cdot)$ and $h_2(\cdot)$ via $\lambda$ to determine the importance between the HJI-VI and the ground truth value function.


 A three-layer DNN with a hidden layer size of 512 neurons is trained using the loss function \eqref{eq:loss_function}. From $V_\theta(r,t;\beta)$, the TEB can be queried at the convergence time in the relative space. We denote the converged parameterized value function as $V_{\theta}^\infty(r;\beta)$. For simplicity, the parameter state queried will represent both $\beta_1$ and $\beta_2$, meaning $\beta_1 = \beta$ and $\beta_2 = \beta$.

 \begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{figures/combined.jpg}
    \caption{(Left) tracking error bounds for a 6D Dubin's car relative system with different planner control bounds $\beta$. Training parameters: 40k pre-train iterations, followed by 110k training iterations. The training stops when the convergence threshold is met. Total training took 10h32m on a NVIDIA A30. As the planner control ($\beta$) increases, the error bound associated with tracking the planner grows larger. (Right) comparison between standard dynamic programming based HJ reachability (using codebase HelperOC) and DeepReach. Empirically, we see that DeepReach produces more conservative error bounds. \vspace{-1.5em}} 
    \label{fig:1}
\end{figure}

\shnote{Introduce figure, discuss.\vspace{8em}} 

We generated probabilistic guarantees for this trained value function. By sampling 36M states within the value function and running the scenario optimization algorithm to 7 iterations, we found the violation rate to be $3.2 \times 10^{-5} << \epsilon$.



\noindent \textbf{Static and Dynamic TEB.} In Parametric FaStrack, we also define two new terms for the TEB: dynamic TEB (dTEB) and static TEB (sTEB). 
The dynamic tracking error bound dTEB is the error bound that is achieved when the planner is navigating through the environment at a current planner control value $\beta$. As the planner changes its speed, this control value (and therefore the dTEB) will change accordingly. Intuitively, as the planner control increases, the TEB expands due to higher variability in the tracking. 

The dTEB in the planner space can be computed as the minimal level set of the value function at a particular $\beta$, i.e. 
$\TEB_{e,d}^\infty(\beta) := \{e: \exists \eta \text{ s.t. }\valfunc_\theta^\infty(e,\eta; \beta) \leq \minval_\theta ^\infty \}$. Recall in the original FaSTrack work that the relative system is defined as $r = (e,\eta)$, where $e$ and $\eta$ are the error and auxiliary states. Without Parameterizing the value function, the dTEB would have to be obtained through several reachability computations via dynamic programming (as done in \cite{fridovich2018planning}), which is computationally expensive and even infeasible for high dimensional systems. 

The sTEB is the error bound that is achieved when the planner is navigating through the environment \textit{as slowly as possible}, i.e. at its minimum control bound $\beta_l$. The sTEB can be computed as the minimal level set of the value function, $\TEB_{e,s}^\infty := \{ e: \exists \eta \text{ s.t. }\valfunc_\theta^\infty(e,\eta; \beta_l) \leq \minval_\theta ^\infty \}.$ 
 In the running example, we associate the sTEB as the smallest control invariant set associated with $\beta_l = 0.5$.


% The sTEB and dTEB in the planner space for the time-varying value function can be obtained by projecting away $\eta$:
% \begin{align*}
%     \TEB_{e,s}(\tau) := \{ e: \exists \eta \text{ s.t. }\valfunc_\theta(e,\eta, t_f - \tau; \beta_l) \leq \minval_\theta \}, \quad \TEB_{e,d}(\tau;\beta) := \{e: \exists \eta \text{ s.t. }\valfunc_\theta(e,\eta, t_f-\tau; \beta) \leq \minval_\theta \}. 
% \end{align*}
% The sTEB and dTEB in the planner space are: 
% \begin{align*}
%     \TEB_{e,s}^\infty := \{ e: \exists \eta \text{ s.t. }\valfunc_\theta^\infty(e,\eta; \beta_l) \leq \minval_\theta ^\infty \}, \quad \TEB_{e,d}^\infty(\beta) := \{e: \exists \eta \text{ s.t. }\valfunc_\theta^\infty(e,\eta; \beta) \leq \minval_\theta ^\infty \}. 
% \end{align*}




%Left figure of Figure \ref{fig:2} outlines the offline framework of Parametric FaSTrack. 


\noindent \textbf{Tracking Controller.} The tracking controller given the relative states can be computed as in \eqref{eq:tracking_control} from the parameterized value function evaluated at the current value of $\beta$.%through its spatial gradients, which will always try to minimize the TEB between the tracking and the planning systems, regardless of the given planner control bound.

